Satisficing and Optimal Generalised Planning via Goal Regression (Extended Version)

Generalised planning (GP) refers to the task of synthesising programs that solve families of related planning problems. We introduce a novel, yet simple method for GP: given a set of training problems, for each problem, compute an optimal plan for each goal atom in some order, perform goal regression on the resulting plans, and lift the corresponding outputs to obtain a set of first-order $\textit{Condition} \rightarrow \textit{Actions}$ rules. The rules collectively constitute a generalised plan that can be executed as is or alternatively be used to prune the planning search space. We formalise and prove the conditions under which our method is guaranteed to learn valid generalised plans and state space pruning axioms for search. Experiments demonstrate significant improvements over state-of-the-art (generalised) planners with respect to the 3 metrics of synthesis cost, planning coverage, and solution quality on various classical and numeric planning domains.

==> support/aaai.tex <==
% !TEX root =moose.tex

\usepackage{aaai2026}  % DO NOT CHANGE THIS
\usepackage{times}  % DO NOT CHANGE THIS
\usepackage{helvet}  % DO NOT CHANGE THIS
\usepackage{courier}  % DO NOT CHANGE THIS
\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\frenchspacing  % DO NOT CHANGE THIS
\setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS

\setcounter{secnumdepth}{2} % Set section numbering depth


==> support/admin.tex <==
%%%%% Original commenting macros
\newcommand{\Todo}[1]{{{\color{red}TODO \emph{#1}}}}
\newcommand{\colourdc}{purple}
\newcommand{\dc}[1]{{\color{\colourdc} #1}}
\newcommand{\till}[1]{\textcolor{teal}{#1}}
\newcommand{\dchide}[1]{{}}
\setlength\marginparwidth{15mm}
\newcommand{\todocustom}[3]{\todo[linecolor=#2,backgroundcolor=#2!25,bordercolor=#2,#3]{#1}}

\newcommandx{\nbdc}[2][1=]{\todocustom{#2}{\colourdc}{#1,size=\tiny}}
\newcommandx{\nbdchide}[2][1=]{}

%%%%% New from Sheila
\newcommand{\showme}[1]{{\color{magenta} #1}}
\newcommand{\notes}[1]{{\color{cyan} #1}}
\newcommand{\revisit}[1]{{\color{blue} #1}}
\newcommand{\added}[1]{{\color{red} #1}}
\newcommand{\alt}[1]{{\color{brown} $\backslash$#1}}
\newcommand{\remove}[1]{{\color{green} #1}}
\newcommand{\removeifneeded}[1]{{\color{cyan} #1}}
\newcommand{\removehide}[1]{}
\newcommand{\todosm}[1]{\textcolor{blue}{({\bf SM TODO:} #1)}}

 \newcommand{\nocommentsm}[1]{}
 \newcommand{\addCRC}[1]{}

%%%%%%%%%%%%%   COMMENTS  %%%%%%%%%%%%%%
%%%%%%%%  TURN COMMENTS ON AND OFF WITH \commentstrue AND \commentsfalse BELOW %%%%%%%%%%%%%%%%

\ifcomments

    % \newcommand{\generalComment}[3]{\textcolor{#1}{({\bf #2}: #3)}}  % Sheila's original comment command
    \newcommand{\generalComment}[3]{\todocustom{{\bf #2}: #3}{#1}{inline,size=\small,caption={}}}  % todonotes to differentiate comments and text

    \newcommand{\commentsmbox}[1]{\generalComment{orange}{SM}{#1}}
    \newcommand{\commentsmboxhide}[1]{}

    \newcommand{\commentsm}[1]{\textcolor{orange}{({\bf SM:} #1)\\}}
    \newcommand{\commentsmhide}[1]{}

    \newcommand{\commenttkinline}[1]{\textcolor{cyan}{({\bf TK:} #1)\\}}
    \newcommand{\commenttk}[1]{\textcolor{cyan}{({\bf TK:} #1)\\}}
    \newcommand{\commenttkhide}[1]{}
    
    \newcommand{\commentdcinline}[1]{\textcolor{\colourdc}{({\bf DC:} #1)\\}}
    \newcommand{\commentdc}[1]{\textcolor{magenta}{({\bf DC:} #1)\\}}
    \newcommand{\commentdchide}[1]{}
    
    \newcommand{\commentth}[1]{\textcolor{teal}{({\bf TH:} #1)\\}}
    \newcommand{\commentthhide}[1]{}


\else

    \newcommand{\commentsm}[1]{}
    \newcommand{\commentsmhide}[1]{}
    
    \newcommand{\commentsmbox}[1]{}
    \newcommand{\commentsmboxhide}[1]{}

    
    \newcommand{\commenttk}[1]{}
    \newcommand{\commenttkhide}[1]{}
    
    \newcommand{\commentdc}[1]{}
    \newcommand{\commentdchide}[1]{}
    
    \newcommand{\commentth}[1]{}
    \newcommand{\commentthhide}[1]{}

    \renewcommand{\nbdc}[2][1=]{}
    \renewcommand{\todo}[1]{}
    \renewcommand{\colourdc}{black}

\fi


==> support/coverpage.tex <==
% !TEX root =moose.tex

\subsection*{Coverpage\\
\footnotesize{(generated by \texttt{support/coverpage.tex} input in \texttt{moose.tex})}}

\subsection*{Macros}
\begin{itemize}
  \item macros are in the file \texttt{support/admin.tex}
  \item \dc{$\backslash$dc looks like this} \commentdc{$\backslash$commentdc looks like this} \commentdcinline{$\backslash$commentdcinline looks like this}
  \item $\backslash$commentdc\{blah blah\} respectively $\backslash$commenttl\{\} etc  creates a comment in a colour.  You're already using "todo" so perhaps this is redundant.
  \item $\backslash$commentdchide\{blah blah\} hides the "blah blah"
  \item $\backslash$remove \remove{turns text light green indicating it's a candidate for removal if we need space}
  \item $\backslash$removehide hides the text
  \item $\backslash$removeifneeded \removeifneeded{highlights text in cyan that is a candidate for removal if we need space (or for some other reason).}
  \item $\backslash$revisit \revisit{turns text blue indicating it's something to reconsider/check -- good for things you're uncertain about or that someone things might be inaccurate/incorrect and warrants discussion}
  \item $\backslash$alt \alt{turns text brown and is an alternative phrasing to what preceded it}
  \item $\backslash$added \added{turns text red to highlight new text that was added --- good in final stages when people are making changes they want others to note/approve/check}
\end{itemize}
Some of the macros:
{\small
\begin{verbatim}
\newcommand{\notes}[1]{{\color{cyan} #1}}
\newcommand{\revisit}[1]{{\color{blue} #1}}
\newcommand{\added}[1]{{\color{red} #1}}
\newcommand{\alt}[1]{{\color{brown} $\backslash$#1}}
\newcommand{\remove}[1]{{\color{green} #1}}
\newcommand{\removeifneeded}[1]{{\color{cyan} #1}}
\newcommand{\removehide}[1]{}
...
\end{verbatim}
}

\vfill
\pagebreak

\setcounter{page}{1}


==> tables/coverage-combined.tex <==
\begin{tabularx}{\tabWidth}{l *{3}{Y} l *{5}{Y} l *{5}{Y}}
  Domain
  & \header{\enhspMQ{}}
  & \header{\enhspHMRPHJ{}}
  & \header{\moose{}}
  &
  Domain
  & \header{\lama{}}
  & \header{\slearnerA{}}
  & \header{\slearnerB{}}
  & \header{\slearnerC{}}
  & \header{\moose{}}
  &
  Domain
  & \header{\blind{}}
  & \header{\lmcut{}}
  & \header{\scorpion{}}
  & \header{\symk{}}
  & \header{\moose{}}
  \\
  \cmidrule(l){1-1}
  \cmidrule(l){2-4}
  \cmidrule(l){5-5}
  \cmidrule(l){6-10}
  \cmidrule(l){11-11}
  \cmidrule(l){12-16}
  NAd & 32 & 23 & \first{90} &
  Ba & 49 & 0 & 0 & 0 & \first{90} &
  Ba & 0 & 0 & 0 & 12 & \first{26} \\
  NCh & 64 & 49 & \first{90} &
  Ch & 35 & 0 & 66 & 0 & \first{90} &
  Ch & 9 & 9 & 9 & 15 & \first{17} \\
  NFe & 60 & 61 & \first{90} &
  Fe & 69 & 67 & 67 & 60 & \first{90} &
  Fe & 10 & 18 & 17 & 18 & \first{30} \\
  NMi & 63 & 71 & \first{90} &
  Lo & 77 & 0 & 0 & 0 & \first{89} &
  Lo & 8 & 15 & \first{22} & 10 & 16 \\
  NMi & 30 & 68 & \first{90} &
  Mi & \first{90} & \first{90} & \first{90} & \first{90} & \first{90} &
  Mi & \first{30} & \first{30} & \first{30} & \first{30} & \first{30} \\
  NTr & 45 & 64 & \first{90} &
  Ro & 66 & 0 & 0 & 0 & \first{90} &
  Ro & 15 & 17 & 18 & \first{20} & \first{20} \\
%   \cmidrule(l){1-1}
%   \cmidrule(l){2-4}
  $\sum$ (540)
  & 294 & 336 & \first{540} &
  Sa & 89 & 0 & 47 & 48 & \first{90} &
  Sa & 12 & 22 & \first{26} & 21 & 21 \\
  & & & &
  Tr & 66 & 0 & 63 & 46 & \first{90} &
  Tr & 9 & 9 & \first{20} & 13 & 15 \\
%   \cmidrule(l){5-5}
%   \cmidrule(l){6-10}
%   \cmidrule(l){11-11}
%   \cmidrule(l){12-16}
  & & & &
  $\sum$ (720)
  & 541 & 157 & 333 & 244 & \first{719} &
  $\sum$ (240)
  & 93 & 120 & 142 & 139 & \first{175} \\
\end{tabularx}
